V-MIND: Building Versatile Monocular Indoor 3D Detector with Diverse 2D Annotations

The field of indoor monocular 3D object detection is gaining significant attention, fueled by the increasing demand in VR/AR and robotic applications. However, its advancement is impeded by the limited availability and diversity of 3D training data, owing to the labor-intensive nature of 3D data collection and annotation processes. In this paper, we present V-MIND (Versatile Monocular INdoor Detector), which enhances the performance of indoor 3D detectors across a diverse set of object classes by harnessing publicly available large-scale 2D datasets. By leveraging well-established monocular depth estimation techniques and camera intrinsic predictors, we can generate 3D training data by converting large-scale 2D images into 3D point clouds and subsequently deriving pseudo 3D bounding boxes. To mitigate distance errors inherent in the converted point clouds, we introduce a novel 3D self-calibration loss for refining the pseudo 3D bounding boxes during training. Additionally, we propose a novel ambiguity loss to address the ambiguity that arises when introducing new classes from 2D datasets. Finally, through joint training with existing 3D datasets and pseudo 3D bounding boxes derived from 2D datasets, V-MIND achieves state-of-the-art object detection performance across a wide range of classes on the Omni3D indoor dataset.

==> figure/supp_class_stat.tex <==
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=0.97\textwidth]{figure/src/supp_class_stat.pdf}
    \caption{\textbf{Per class training data distribution.} The bar chart presents the number of 3D boxes of the Omni3D~\cite{omni3d} indoor dataset and the lifted LVIS~\cite{gupta2019lvis} data on a logarithmic scale. 
    %
    The original classes, ranging from \textit{chair} to \textit{bicycle}, and the new classes, from \textit{toys} to \textit{printer}, are shown on the x-axis. 
    %
    Our generated data from the LVIS~\cite{gupta2019lvis} dataset spans a wide range of object categories, with a substantial number of 3D pseudo bounding boxes.
    }
    \label{fig:class_stat}
\end{figure*}

==> figure/supp_lvis_pseudo_box.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.47\textwidth]{figure/src/supp_lvis_pseudo_box.pdf}
    \caption{\textbf{Qualitative results of the 3D pseudo bounding boxes lifted from the LVIS\cite{gupta2019lvis} 2D dataset.}
    The pseudo boxes are accurate in both their sizes and 3D positions.
    }
    \label{fig:supp_lvis_pseudo_box}
\end{figure}

==> figure/supp_qualitative.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.98\textwidth]{figure/src/supp_qualitative.pdf}
    \caption{\textbf{Qualitative results of {\ours} and baseline Cube R-CNN.}
    Through our proposed method, {\ours} has the ability to detect a wider range of object classes in 3D.
    %
    For example, the monitor and keyboard in the first row, as well as the microwave and toaster in the second row, are all new classes that are not present in the human-annotated 3D training data. 
    %
    This demonstrates the effectiveness of our proposed method.}
    \label{fig:supp_qualitative}
    
    \vspace*{15pt}
\end{figure*}

==> table/3d_detection.tex <==
\begin{table}[t]
\small
\centering
\caption{
  \textbf{3D object detection result on Omni3D indoor subset}.
  \vspace{5pt}
}

\begin{tabular}{lcc}
\toprule
     & AP\textsubscript{3D} \\ \midrule
Ours & 13.98                \\
\bottomrule
\end{tabular}

\label{table:3d-detection}
\end{table}


==> table/supp_filtering_stat.tex <==
\begin{table*}[!htb]
% \small
\centering
\caption{
    \textbf{The statistics of the number of pseudo boxes at different stages of the filtering process for the LVIS~\cite{gupta2019lvis} dataset}.
    The negative numbers indicate the \textit{reduction} in the number of pseudo boxes at each filtering stage.
    %
    Since our paper focuses on indoor object detection, the majority of boxes are filtered out during class filtering as they correspond to outdoor categories.
}

\begin{tabular}{l|c|ccc|c}
\toprule
                          &  Original \#boxes &  Class filtering  &  Cube R-CNN filtering~\cite{omni3d}  &  Point filtering  &  Final \#boxes   \\ \midrule
LVIS~\cite{gupta2019lvis} &  790,884   &  -459,840         &  -80,191             &  -87,165         &  163,688       \\
\bottomrule
\end{tabular}

\label{table:filter_stat}
\end{table*}

==> table/supp_img_anno_stat.tex <==
\begin{table}[!htb]
% \small
\centering
\caption{
    \textbf{The statistics of the training data for each dataset}. 
    We include only the training split of the LVIS~\cite{gupta2019lvis} dataset for our pseudo data generation.
    %
    The ARKitScenes~\cite{dehghan2021arkitscenes} and Hypersim~\cite{hypersim} are multi-view datasets, where many duplicate images and boxes represent the same scenes.
    %
    Additionally, the Hypersim is a synthetic dataset, making it easier to generate large amounts of data but prone to domain gaps.
    %
    In contrast, the data we generate from the 2D LVIS dataset is real-world, diverse, and contains a substantial number of instances.
}
\resizebox{0.47\textwidth}{!}
{
\begin{tabular}{l|rr|rr}
\toprule
\multicolumn{1}{l}{}      & \multicolumn{2}{c}{\#Images}  & \multicolumn{2}{c}{\#Boxes} \\ \midrule
                          &  Train  &  Val   &  Train    &  Val   \\ \midrule
LVIS~\cite{gupta2019lvis} &  48,759 &  -     &  163,688  & -      \\
SUN-RGBD~\cite{SUNRGBD}   &  4,639  &  333   &  18,913   & 1,321  \\
ARKitScenes~\cite{dehghan2021arkitscenes}    &  43,687   & 4,791 &  95,730 & 10,945 \\
Hypersim~\cite{hypersim}  &  48,978 &  6,738 &  674,206  & 75,046 \\
\bottomrule
\end{tabular}
}
\label{table:img_anno_stat}
\end{table}
